Rational Threshold Cryptosystems

We propose a framework for threshold cryptosystems under a permissionless-economic model in which the participants are rational profit-maximizing entities. To date, threshold cryptosystems have been considered under permissioned settings with a limited adversary. Our framework relies on an escrow service that slashes and redistributes deposits to incentivize participants to adhere desired behaviors. Today, more than ever, sophisticated escrow services can be implemented over public blockchains like Ethereum, without additional trust assumptions. The key threat to rational threshold cryptosystems is collusion---by cooperating `illegally', a subset of participants can reveal the cryptosystem's secret, which, in turn is translated to unfair profit. Our countermeasure to collusion is framing. If the escrow is notified of collusion, it rewards the framer and slashes the deposits of all other participants. We show that colluding parties find themselves in the prisoner's dilemma, where the dominant strategy is framing.

==> GJKR.tex <==
\steven{This is still background}
In this section we outline the GJKR-DKG protocol \cite{DKGRevisited} for discrete-log based threshold cryptosystems. The protocol was first introduced by Pedersen in~\cite{PedersenDKG}. In a following work~\cite{DKG}, Gennaro et al. found a vulnerability and suggested to mitigate it via an additional communication phase. Later, in~\cite{DKGRevisited}, they returned to the original Pedersen protocol and proved its correctness under relaxed (but practical) requirements. We begin with the model and then describe the protocol and its properties.

\subsubsection{Model.}
The protocol is run among a set of $n$ (known) \emph{participants} $P_1,\dots,P_n$, which are modeled as probabilistic polynomial time Turing machines. We assume the existence of an \emph{adversary} that can corrupt up to $t$ of the players and control their behavior.

\paragraph{Communication.}
Communication in the protocol is assumed to be \emph{synchronous}, that is, a message is delivered from source to destination within some known and fixed time bound. The participants may use private communication channels or a public broadcast channel. For private communication, a complete network of encrypted and authenticated point to point channels~\cite{DKGRevisited} is assumed to allow any two participants to communicate privately. For messages sent via the public broadcast channel, it is assumed that the data received is consistent among \textbf{all} participants. In particular, every participant should be convinced that the data they received via the public broadcast channel matches the data received by others.

\paragraph{Adversary.} \label{adversary}
The adversary $\mathcal{A}$ can corrupt up to $t<n/2$ participants. $\mathcal{A}$ is \emph{static} in the sense that it chooses the participants it corrupts at the beginning of the protocol. The adversary does not have additional computational capacity over that of the participants it corrupted and is also modeled as a probabilistic polynomial time Turing machine. The adversary is assumed to be {\em malicious}, meaning corrupted participants may arbitrarily deviate from the protocol. We make no limiting assumptions about the goals of the adversary which may include causing the protocol to fail and learning information about secret values.
    
\subsubsection{Protocol Description.}
Recall that, informally, the goal of a $(t,n)$-DKG protocol is twofold---abstractly generate a global secret key (although it is never constructed or known by any entity), and distribute key shares that jointly correspond to the global secret. Any $t+1$ key shares can reconstruct the global secret, but $t$ (or fewer) key shares cannot be used to extract any useful information.
%\red{about} it (this is crucial since the adversary can corrupt up to $t$ participants). 

These goals are easy to achieve if a trusted dealer is present. In the spirit of Shamir's secret sharing~\cite{SecretSharing}, \steven{You need to put Shamir in the background before referring to it here. basically put the next two sentences earlier under a heading for SSS} the dealer would generate a degree $t$ polynomial $f$, and share with $P_i$ her secret key share $f(i)$. Then, the reconstruction could be done using Lagrange interpolation, where the global secret is $f(0)$. Feldman~\cite{FeldmanVSS} showed how this procedure could be made \emph{verifiable}, allowing the participants to verify the validity of their key shares. 

Pedersen~\cite{PedersenDKG} was the first to design a DKG protocol achieving the above goals without a trusted dealer. His protocol, \emph{Ped-DKG}, consists of $n$ parallel Feldman VSS runs, each led by a participant $P_i$ sharing a ``local'' polynomial $f_i$. The global polynomial $f$ is defined to be the sum of the local polynomial. The protocol relies on the fact that the sum is taken only on those polynomials which were shared correctly, which is crucial to the success of the protocol. This set is referred to as the set \emph{QUAL} of ``qualified'' polynomials.

Gennaro et al. point out a last actor attack in Ped-DKG, giving the adversary some control over the composition of the set QUAL. In \cite{DKG} they mitigate this problem using an additional communication round to construct QUAL properly, and in a later work~\cite{DKGRevisited} they prove that under relaxed (yet practical) requirements, the original Ped-DKG is sufficient. 

The full description of Ped-DKG is given in \red{the appendix} \red{Fig.~\ref{FigGJKR}}.

\subsubsection{Protocol Properties.} \label{properties}
\steven{remove next sentence. it doesn't convey useful information} Defining the requirements from a DKG protocol is not a trivial task. In their papers, Gennaro et al. formulate a minimal set of requirements for a $(t,n)$-DKG protocol in Discrete-Log based cryptosystems. 

\paragraph{Correctness.}
\begin{itemize}
\item[(C1)] There is an efficient procedure that on input any $t+1$ (distinct) secret key shares produced by the protocol, outputs the same secret $x$. There is another efficient procedure that on input \steven{this doesn't have to be n right? n could be really large and you dont need all of them to get this property} $n$ secret key shares (of which at least $t+1$ were produced by the protocol) and the public data produced by the protocol, outputs the unique global secret $x$\footnote{Note that the requirement $t<n/2$ in~\ref{adversary} guarantees that among the $n$ submitted key shares, at least $t+1$ of them are correct \steven{in the honest majority setting}.}.

\item[(C2)] There is an efficient procedure that on input the public data produced by the protocol, outputs $g^x$, where $x$ is the unique secret key guaranteed by (C1). \steven{why not just say: The protocol outputs the public $g^x$, where $x$ is the shared secret}

\item[(C3)] $x$ is uniformly distributed in $Z_q$, hence $g^x$ is uniformly distributed in $G$. \steven{Is the distribution a correctness property?}
\end{itemize}

\paragraph{Secrecy.} 
No information on $x$ can be learned by the adversary except for what is implied by the value $g^x$. A more formal description of the secrecy property involves a simulator which mimics \steven{more specifically, produces a transcript from the same distribution} the output of the DKG protocol based on $g^x$ alone. \red{This should be rephrased later somewhere in more general terms---no adversary and not necessarily $x$.}




%More formally, for every probabilistic polynomial time adversary $\mathcal{A}$, there exists a probabilistic polynomial time simulator $SIM$, such that on input an element $y\in G$, produces an output which is polynomially indistinguishable from $\mathcal{A}$'s view of a run of the DKG protocol that ends up with public key $y$ and in which $\mathcal{A}$ corrupts at most $t$ participants.

The protocol presented in~\ref{FigGJKR} achieves properties $(C1)$, $(C2)$. The attack presented in~\cite{DKG} is shown to compromise $(C3)$, which also breaks the standard proof of the secrecy property. The protocol we present in Sec.~\ref{} is very similar to Ped-DKG, but we solve the above attack using hash commitments. \steven{here's where you should highlight the fact that they don't check the group. say something like: we also point out and correct a problem in their protocol which makes their security proof fail. You also want to highlight this in the introduction}

%\red{In their later work~\cite{DKGRevisited} the original protocol is reconsidered and the last actor problem is circumvented by considering a slightly weaker (but still practical) set of required properties and a more involved simulator proof. It is shown that the protocol suffices to distribute key shares for an unforgeable threshold Schnorr signature scheme.}

While we omit the proofs from~\cite{DKGRevisited} and \cite{DKG}, we note that they rely on similar properties satisfied by Feldman VSS with a \textbf{single} dealer. \red{For completeness, we present these properties in the appendix.}

%The correctness and secrecy properties in \red{Ped-DKG/Joint-Feldman} (Fig.~\ref{FigGJKR}) rely on similar properties in Feldman's VSS with a \textbf{single} dealer. In a Joint-Feldman protocol every participant serves as a dealer, and the proofs for Feldman's VSS properties can be easily generalized. 



\subsubsection{Discussion.}
While theoretically Joint-Feldman DKG provides correct and secret keys, it suffers several practical drawbacks. We discuss these briefly, alluding to our modifications.

\paragraph{Adversarial model.}
Lacking an adversary, a DKG protocol can be made trivial. The complications appear when the protocol should \red{admit} certain properties when an adversary does exist. Assuming an adversary implies there is something to gain from interrupting with the protocol. The Joint-Feldman approach lacks a clear notion of this ``gain''. \red{However, in order to have a functioning system, the adversary must be limited---the protocol relies on the adversary corrupting at most $t$ players. Quite ironically, an adversary controlling $t$ players is unlikely to stop there as she is highly motivated to corrupt the $t+1$ player and get control of the underlying cryptosystem.}

The key element that enables us to define an economical model is a trusted, publicly available escrow service that can enforce a general set of rules---the Ethereum blockchain can be used to implement such a service.

\paragraph{Complaints and the set QUAL.}
The complaint mechanism in Ped-DKG relies on the fact that a player can reveal up to $t$ of her sub-shares (points on her secret polynomial) without breaking its secrecy. This is of course theoretically true, but weakens the security-guarantees of the protocol. Imagine a situation where player $P_i$ has revealed $t$ of her sub-shares (due to $t$ complaints against her). Without loss of generality, let those be $f_i(1), \dots, f_i(t)$. Now, in order to reveal $f_i$, it suffices to hack \textbf{any} of the players that did not complain, i.e., $P_{t+1}, \dots, P_n$. This is a much easier task then having to hack specifically $P_i$.
 
\steven{I didn't understand this paragraph. We said in the model that we don't assume any limitations to the goals of the attacker, so I'm not sure if this is really strengthening the attack}Another issue is that more than $t$ participants can coordinate their complaints to exclude other participants from the set QUAL. This opens the opportunity to influence the secret (or the polynomial $f$) and may serve as further motivation to get control of $t+1$ players over the general motivation of acquiring ``full rights'' in the underlying cryptosystem. 

\paragraph{Public broadcast channel.} 
Finally, while the theoretical papers \steven{don't say ``the theoreetical papers'' insted just cite them --i.e. while \cite{foo,bar} assume...} assume the existence of a reliable broadcast channel, implementing one is a considerable hurdle. The difficulty boils down to the fact that reliable broadcast amounts to reaching consensus in an adversarial environment. Consensus protocols are quite complicated---they introduce the need for participant authentication (e.g., MACs or digital signatures), require extra communication rounds, do not scale well in the number of participants, and in asynchronous networks restrict the bound on the faulty participants to $t<n/3$\red{~\cite{ThirdBoundBFT}, verify citation}. As discussed in the background, public blockchains, and specifically Ethereum, emerge as reliable broadcast mediums that meet the needs of a DKG protocol in the spirit of Joint-Feldman.

%\red{As a matter of fact, a simple enhancement of GJKR would come in the form of the participants having some kind of public-key identity and signing capabilities. This would highly reduce the difficulty of arbitration as complaining participants could provide proof of non-valid sub-shares they received in the form of signed messages. Ethereum can readily enhance GJKR in this regard, but it has a significant additional advantage---it can serve as \emph{the} arbitrator and can thus serve as an escrow as well, slashing whoever is detected as malicious.}

%Before heading on, we exemplify the importance of public broadcast via the following simple attack. Lacking a reliable broadcast channel, $P_i$ is able to convince $P_j$ in one set of commitments $X_{i,k}$ and the others in a different set $Y_{i,k}$. $P_i$ sends $P_j$ the sub-share $x_{i,j}$ corresponding to $X_{i,k}$, and the others the sub-shares $y_{i,k}$ corresponding to $Y_{i,k}$. Since in the view of each participant the sub-shares are consistent with the commitments, no complaint would be filed and $P_j$ would be left with a useless key-share. In particular, property $(C1)$ would not hold.

\paragraph{}In the next section we discuss our variant of the original Ped-DKG protocol. Our economic driven model applies to both the DKG protocol as well as once the key generation has been completed and the threshold cryptosystem is being used. Thus, we regard the DKG and the underlying threshold cryptosystem as one complete system.









==> Old.tex <==
\red{Just some thoughts: Let's examine a few possible scenarios. If at least $1$ node and less than $t+1$ participants complain against a specific node, she must be considered correct, as no unambiguous decision can be made. She would be asked to reveal her shares via the public channel, but would remain in the set QUAL. Otherwise, she is excluded from the protocol as she must be corrupted. 
Additionally, if at least $t+1$ participants are complained against then at least one complainer must be corrupted. If less than $t+1$ nodes remain the protocol must fail as it might be the case that only corrupted nodes are actively contributing to the scheme's secret which means they know everything.
Another thing, it is necessary that $t+1$ honest nodes do participate, that is $n \geq 2t+1$. Otherwise, .....
In essence, a correct participant can be defined as one whose commitments are consistent with the \emph{whole} set of sub-shares she sent the other participants. Since sub-shares are distributed privately between pairs it is generally hard to determine who is lying in case of a dispute. In GJKR, this is solved without the need of digital signatures but with strong assumptions on the communication channels and the active participation of the honest, complaining whenever they detect a mismatch. Another approach could use digital signatures, providing proof a node has sent a non-valid sub-share, reducing the complexity of the arbitration process in GJKR. The problem of putting the protocol to a halt at no cost would still stand. Using Ethereum is yet another approach that incentivizes correct participation and discourages halting the protocol.   
The property we wish to verify is: a participant is included in QUAL if and only if her commitments are consistent with the sub-shares she sent to the other participants. This mechanism heavily relies on the assumption that there are no more than $t$ adversarial participants: \red{they} consider any statement made by $t+1$ participants as true. This allows the protocol to detect faults \textit{and} cleverly correct them within the run of the protocol, such that the protocol \emph{always} terminates successfully.          
Instead of relying on this sort of consensus, we rely on the Ethereum computation power to unambiguously decide whether a filed complaint is justified or not. This tool allows us to implement a cryptoeconomic driven complaint mechanism in which any single complaint can be checked and invoke an (economic) punishment (complaints thus must be verifiable). It works as follows:}
\red{describe the mechanism---filing complaints, invoking computation on Ethereum, slashing.}

Our complaint mechanism results is different from the one of GJKR in three essential aspects: 
\begin{enumerate}
\item Our protocol always detects the identity of the incorrect participant, as well as the nature of its incorrect statement (i.e., dealt inconsistent shares). 
\item Participants are penalized for incorrect behavior: their deposit is slashed and distributed among the correct participants. 
\item Our protocol does not endure faults. \emph{Every} complaint results in the non successful termination of the protocol, with no key generation or shares distribution. 
\end{enumerate}
The zero tolerance implied by the third item presents the risk of the adversary preventing the successful termination of the protocol. However, the slashing allows us to make a \textit{liveness} statement, which we prove in Sec.~\ref{correctnessSecurity}:
\begin{lemma} [Liveness of GJKR*]
\end{lemma}

\red{I want to include this somewhere: What happens if the $t$ assumption breaks? In both protocols, if there is indeed a $t+1$ coalition, then it's of their best interest to comply to the protocol, gaining complete signing rights. That's true simply because they are $t+1$. Even if they are not reconstructing the shared secret or the secrets of the other participants they have full signing rights. However, in the original GJKR protocol they can exclude other participants, controlling the polynomial $f$ and the scheme's secret key (which can be problematic for using it to realize a randomness beacon). Can the bad guys make sure the keys the good guys get are malfunctioning?}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\red{Collusion resistance relates to the cryptosystem as a whole, not only the DKG.}

In the following section we demonstrate collusion resistance in a specific threshold cryptosystem in which the collusion pressure can be measured quantitatively.

Consider $n$ participants in a $(t,n)$-Eth-DKG protocol (with deposit $D$) that distributes keys for a threshold BLS signature scheme and assume the signatures are used in order to repeatedly produce random values every round. That is $RS^r=sig_{t+1}(RS^{r-1})$. Such a randomness beacon can be used for a $R$-round lottery (or card game) in which, in every round, at most $m$ tickets are sold at a fixed price $Y$. For their services, the participants get a certain commission (divided evenly), which is some small percentage $\alpha$ (say $\alpha=0.1$) of the total pot per round $Ym$. 

Our main goal is to design the cryptosystem such that $RS^r$ is not known (to any entity) prior to the end of the ticket sale of round $R$. More accurately, we will show that under the framing mechanism presented above, a lottery can be built in which \red{the dominant strategy} of each participant leads to an equilibrium that keeps the random seed secret until the time comes.

\begin{definition} [Collusion]
A collusion in a $(t,n)$-threshold cryptosystem is said to have occurred if $t+1$ shares have been combined \textbf{before} a designated time.
\end{definition}

Let's examine the possible scenarios in which such a cryptosystem could evolve:

\underline{Happy flow.} The desired behavior of the system is that a DKG participant has no advantage if she were to gamble in the lottery. Put differently, at the time gambler $g$ (any gambler) acquired his ticket, he had no information on the winning ticket (a formal argument could be that given an oracle presenting him with two tickets---the winning ticket and a losing one---he would have $0.5$ chance of getting the winning ticket no matter the strategy he chose). If this was correct, it would deduce that no collusion has taken place, revealing the winning ticket before the sale has ended. In this scenario, the profit expected by a gambler is slightly negative (but the high variance makes it exciting to play). The profit of the DKG participants is simply $\frac{\alpha \cdot R \cdot Ym}{n}$, which is paid to them for the services they give. i.e., producing economically secure randomness by investing $D$ Eth. We shall assume this investment channel is lucrative in order to have participants join---So tuning $\frac{\alpha \cdot R \cdot Ym}{n}$ to around $0.1D$ sounds right (this should \red{include} the risk of being complained against or framed). As an individual DKG participant this would be option a and it would imply refusing joining any coalition of $t+1$ participants.

\underline{Collusion without framing.} The worst result in term of the gamblers is that a collusion indeed happens and the coalition thus wins the winning ticket of every round. First, by designing the protocol correctly we could have the possibility of multiple winning tickets, forcing the coalition to split her rewards from time to time. Another option would be that the coalition cannot buy the winning ticket but only foresee the round's evolution making wise decisions (for example in a poker game, where the coalition knows the pack of cards). Then, she would win only some fraction of the rounds and not all of them. We will make a worst case estimation, assuming the coalition wins every round. That is, every coalition member takes (in addition to her fees from the previous case) a sum of $\frac{(1-\alpha) R\cdot Ym}{t+1}$. In view of the coalition this is the most profitable strategy--- almost all the money in the pile goes to her.

\underline{Collusion with snitching.} \red{We shall show that the most profitable strategy of the coalition is not the dominant strategy in terms of the individual participants.} If indeed the previous scenario were to emerge, each of the $t+1$ coalition members would have the possibility to snitch and get a reward of $t\cdot D$. If $t\cdot D > D + \frac{(1-\alpha) R\cdot Ym}{t+1} + \frac{\alpha \cdot R \cdot Ym}{n}$ it is definitely a better strategy for every member in the coalition to snitch. The fear the snitching mechanism introduces, discourages DKG participants from joining a coalition. As a matter of fact, even if the inequality does not hold she might still be encouraged to snitch as it would mean securing her profit, while in giving up snitching there is much risk---someone else might snitch, or the popularity of the lottery might reduce. Let's write the more accurate condition as: $$t\cdot D > (1-P_s) \big( D + \frac{(1-\alpha)\cdot R\cdot Ym}{t+1} + \frac{\alpha \cdot R \cdot Ym}{n} \big) - P_s D$$ As a matter of fact, if $t\cdot D$ is a relatively large sum of money we could expect snitching in very high probability. 

\underline{Reducing the incentive to snitch.} If the coalition is ``naive'', quite trivially $P_s$ tends to $1$. The coalition thus must discourage its members from snitching. The \red{only} way this could be done (in case the members are rational profit-maximizing entities) is to have them lose more from snitching. The coalition could then build its own smart contract, having each of the members deposit a sum of money $C$. In case of a snitch in the original cryptosystem smart contract, all deposits in the coalition's smart contract would be burnt. As $C$ grows the incentive to snitch reduces, and when $C=t\cdot D$ it completely diminishes. We thus get to the final result---if we believe investing $(t+1)\cdot D$ for a profit of $\frac{(1-\alpha) R\cdot Ym}{t+1} + \frac{\alpha \cdot R \cdot Ym}{n}$ is highly unlikely or that simply the sum $(t+1)\cdot D$ is simply unfeasible to deposit\footnote{If we wanted to consider anonymous enrollment regimes, then it is of high importance that indeed $(t+1)\cdot D$ is unfeasible to deposit to make sure there is not one entity in control of the cryptosystem.}, we could participate as gamblers in this lottery, believing the game is being played fairly. Note that an amazing sum of $(t+1)^2\cdot D$ would have to be deposited.

\underline{Interpreting the equations.} It is quite clear that as we might expect $D$, $n$ and $t$ should be high to increase collusion resistance. However, a bit surprisingly, $\alpha$ could be rather small in this aspect. The only reason why we consider increasing $\alpha$ is to drive participation and motivate participants to share their signature shares when its time. \red{In the full analysis we found a constraint on $\alpha$, as one would expect to find.}   

\red{Let's now consider how the framing mechanism kicks-in. Let's consider the most profitable selfish strategy of a colluder: 
If she does not frame the others (by publishing the valid $RS^r$ before time) and so do non of the other colluders, she is expected to profit (less then) $$ \frac{\frac{t+1}{m}\cdot R \cdot Ym}{t+1}=RY $$ where, $\frac{t+1}{m}$ is the team's winning probability per round (this can also be $1$ in some games), $Ym$ is the winning prize per round and the division by $t+1$ is due to the distribution of the prize among the team. 
Her other option is to frame, in which she would immediately get $tD$. In order to discourage her from framing she would need to lose more than that in case she frames. That would mean she would need to put at risk (somehow, maybe another smart contract) this amount. If $D$ is large enough and $t$ is of order of $n$ (and large enough $n$) this might be too much. If the numbers are tuned correctly, it would be a much less attractive investment channel for her.}

==> background_crypto.tex <==
%\subsubsection*{Discrete-Log Based Cryptography}
%Let $G=\langle g \rangle$ be a cyclic group of order $q$, and $x\in Z_q$ some integer. The \emph{discrete-log problem} (DLP) in $G$ asks to compute $x$ given the pair $(g,g^x)$. Numerous \red{public key} cryptosystems are based on the assumption that in certain groups \red{(of efficient representation, and where $g^x$ can be efficiently computed given $x$ and $g$)}, the DLP is \emph{hard}, namely that no probabilistic polynomial time Turing machine can solve a random instance of the DLP in $G$, except for with negligible probability (see \cite{JouxDLP}). 

%\subsection*{Threshold Cryptography}
Threshold cryptography~\cite{thresholdcrypto} refers broadly to techniques for allowing only \emph{joint groups} of parties to use a cryptosystem, be it to compute signatures, or decrypt ciphertexts. In particular, a $(t,n)$-threshold signature scheme consists of $n$ participants (often called {\em players}), where the cooperation of $t+1$ is necessary in order to sign messages. Security of a threshold signature scheme guarantees that $t$ or fewer participants cannot produce a valid signature.

A threshold cryptosystem \red{(back to general cryptosystems and not signatures)} consists of two stages:  
\begin{enumerate}
\item A key generation executed once to set up a common secret key $x$ corresponding to a public key $X$, as well as secret key shares $x_1,\dots,x_n$ held privately by each participant, together with corresponding (public) verification keys $X_1,\dots,X_n$.  \steven{I'm not sure that the public verification keys belong here.}
\item An application stage, where the key shares may be jointly used over and over in order to sign messages or decrypt data. 
\end{enumerate}
Since the key shares must be related to one another, the key generation stage must be coordinated and cannot be done independently by each participant. In the absence of a trusted coordinator, \emph{Distributed Key Generation} (DKG) protocols allow a set of $n$ participants to jointly distribute key shares, without the secret key $x$ ever being constructed and while maintaining threshold security the entire time.
%Sec.~\ref{} gives a detailed account of a specific DKG protocol presented in \cite{DKG}, designed for general cryptosystems relying on the DLP.



%%%COMMUNICATION CHANNLELS WE WON"T USE:

%\red{This needs to go the proof that our private communication scheme over Ethereum is actually private}    
%\underline{Security of Static Diffie-Hellman.} 
%Reusing random values in Diffie-Hellman schemes is done in practice in various settings and is usually considered dangerous, partly due to the exposure to small subgroups attack (\cite{LimLeeSmallSubgroupsAttack}, \cite{ReusingEphemeralKeysDH} and references therein). However, when the group $G$ is of prime order, this attack is irrelevant. Moreover, research on the hardness of the Static Diffie-Hellman Problem, described and discussed in \cite{StaticDiffieHellmanProblem}, suggests that using a static key across multiple parties as done in our scheme is safe so long as the number of parties $n$ is small enough. The up to date algorithms require $n$ to be approximately $r^{\frac{1}{3}}$. In our setting we consider $n\approx 100$ and in no way more than $10,000$, while $r\approx 2^{256}$. 
    
%While the general belief is that static Diffie-Hellman should be secure in certain limited settings (such as our use-case), up until recently this belief had not been formalized and, as far as we know, no attempt was made to define the required conditions for the security of a static Diffie-Hellman scheme. \red{As a first step in this direction we offer the following definition for static Diffie-Hellman security, and prove that our scheme admits this notion of security.}
    

%\red{This should be part of the proof that our private communication over Ethereum is indeed private.}
%\underline{One-time P.C.C. over Ethereum. \red{Regular}}
%Our scheme is based on the Diffie-Hellman key exchange, using the shared key as a one time pad to encrypt the message $m$. A group $G=\langle g \rangle$ of order $r$ for which the Diffie-Hellman problem is assumed to be hard is chosen and published as a system parameter.
%Every participant $i$ generates $n-1$ random numbers $\xi_{i,j}\in Z_r$ and includes them in its enrollment transaction. The secret key shared by $i$ and $j$ is then $k_{i,j}:=g^{\xi_{i,j}\cdot\xi_{j,i}}$. Since the data published in the smart contract is authenticated (via the Ethereum address of the issuer of the transaction), this key exchange is a valid Diffie-Hellman Key Exchange protocol, resulting in a secret key between each pair of participants. When $i$ wishes to send $j$ a message $m$ privately, it publishes $c:=m\oplus H(i,j,g^{\xi_{i,j}\cdot\xi_{j,i}})$, i.e., sends $c$ to the smart contract.
    
%\underline{Security of P.C.C.} 
%\label{CommSecurity}
%It is clear that a message $m$ which was sent from $i$ to $j$ via the above P.C.C. is readable by $j$. It is left to prove that $m$ is indeed kept secret from all other participants. The argument is as follows. If $c$ is (polynomially) distinguishable from a random $|c|$-bit string, then clearly so is $H(i,j,k_{i,j})$. Since $H$ is a random oracle, knowledge of the output is equivalent to knowledge of the input. However, the input contains the secret $k_{i,j}$ shared by $i$ and $j$ alone (this is by the correctness and security of the Diffie-Hellman key exchange). We conclude that only $i$ and $j$ may have any knowledge on $m$ from $c$, and indeed our scheme may \red{use (use what? This is written badly)} as a private communication channel for the DKG scheme.





    
 

==> correctnessSecurity.tex <==
Our protocol should be viewed as an implementation of the revisited GJKR DKG in a specific crypto-economic setting. As such, we draw the security and correctness properties from those in \cite{DKG} and \cite{DKGRevisited}, and make the necessary additions and modifications.

Due to the complaints and slashing approach, not all runs of the protocol are \emph{successful}, namely, end without any complaint being filed to the smart contract. For this reason, we require the correctness and secrecy properties to hold only in case a successful run of the protocol. However, this approach calls for a \textit{liveness} property to complement the correctness and secrecy. 

\red{Consider: As our protocol utilizes a specific communication protocol , based on Ethereum it is necessary to show it admits to the properties assumed in the original protocol.} Another crucial aspect in proving correctness and security is the communication scheme we utilize, which should admit the properties of being private or public according to the protocol requirements. 

\subsection{Communication}
It is quite straightforward that any data which is published on the smart contract is both public and authenticated (via the Ethereum signatures). Other than that, the data - both private and public - should be sent via private peer-to-peer channels we expect the participants to establish. These channels are assumed to be secure. 

\begin{claim}[private communication]
The DKG* private communication scheme over Ethereum admits the properties of private communication from GJKR. That is, a private message sent from $i$ to $j$ is not tappable by any third party $l\neq j$, but is readable by $j$. And any entity wishing to send a private message can do it within $epoch/2$ blocks.
\end{claim}

\begin{claim}[public communication]
The DKG* public communication scheme over Ethereum admits the properties of public broadcast from GJKR. That is, a public message sent from $i$ is received by all participants in one form. And any entity wishing to publish a message can do it within $epoch/2$ blocks. 
\end{claim}

Actually, our communication scheme handles another issue that the original protocol is not concerned with but may simplify things and reduce the strategy space of corrupted players. The problem of not being able to rule in case of a ``did not hear'' complaint. That is, when participant $j$ claims that she failed to receive some data from $i$ who is faulty? Did $i$ really not send it? Is $j$ lying? Or maybe the network failed. For this scenario we incorporated the \red{\emph{ping} mechanism described in \ref{PingMechanism}}, which was introduced to prevent ambiguity regarding whether or not $j$'s complaint is justified. 

In case the missing data is public, $i$ is requested to simply send the data to the smart contract, making it known to all Ethereum nodes as explained above. We are left with the case of the missing data being private, namely that $j$ claims she did not receive $\bar{x}_{i,j}$. In this case $i$ uses the ElGamal encryption scheme and sends the encrypted message to the smart contract. By the correctness and security of the ElGamal scheme, this ciphertext may only be encrypted by $j$ alone, which proves all private data used in \name is indeed private.

\red{there are issued related to who's paying gas for these transactions, etc. Maybe we should dedicate a subsection for incentives etc.}

% \underline{Public Communication}
% \begin{claim}
% 	If $i$ follows the protocol, then all data which $i$ publishes at phase $kl$ using the public communication scheme is indeed accessible to all participants within the time frame of that phase.
% \end{claim}
% \underline{Private Communication}
% \begin{claim}
% If $i$ and $j$ both follow the protocol, then data which is defined in \name as private at phase $l$ is indeed private, i.e., known only to the issuer of the data $i$ and the recipient $j$, within the time frame of that phase. 
% \end{claim}
% \begin{proof}

% \end{proof}

\subsection{Correctness, Secrecy and Liveness}
\red{Should all those be together?}
The correctness and security of our protocol are derived from the correctness and security of the GJKR protocol. The essential difference between the protocols lies in the compliant mechanism, in which we use the smart contract computation instead of the consensus mechanism in GJKR. In our protocol a successful run is very easy to analyze in terms of correctness and security. And so, the core of this section is to prove the liveness property. To define it precisely, we give a complete detailed account of all possible ways in which participants may deviate from the protocol.

\paragraph{Economic concerns.}
It is implied from our model that the \red{only} strategy participants may follow is one in which they cannot be slashed. Thus, the only misbehavior they may consider is not filing a complaint when such is detected. However, if they do, they get a reward of $D/2$. The adversary would have to pay the node more than that. If we can estimate correctly the economical power of the adversary we can choose the parameters to conclude with a setting that matches the original model's assumptions.

\red{We have discussed qualitatively what `being corrupted' means---not following the protocol's rules. Now, that we have seen the protocol we can  explicitly list all the possible misconducts that a node can perform.}

\begin{definition}[Faulty participants.]
A participant who acts not according to protocol is said to be faulty. Explicitly, a participant $i$ is faulty if \red{it preformed at least one of the following misconducts.}
\begin{enumerate} \label{FaultyList}
\item Did not publish the data for a specific phase before the timeout of that phase.
\item Published an encryption public key $pk$ which is not in $\Gamma$. 
\item Sent a commitment which failed group membership test, i.e. $X^u_{i,k}\notin G_u$ for some $u\in \{1,2\},k\in \{0,\dots,t\}$.
\item Published a set of commitments which do not match the Merkle root she published on Ethereum, or that $X^u_{i,0}$ does not match the hash commitment she published in her enrollment transaction. 
\item Published two commitments $X^1_{i,k_0},X^2_{i,k_0}$ which are inconsistent with one another, i.e. $e\big(g_1,X^2_{i,k_0}\big)\ne e\big(X^1_{i,k_0},g_2\big)$.
\item Sent a sub-share $\bar{x}_{i,j}$ which is inconsistent with her commitments, i.e., $g_u^{\bar{x}_{i,j}}\ne \prod_{k=0}^t\big(X^u_{i,k}\big)^{j^k}$ for some $u\in \{1,2\}$. Notice this includes both the regular case of a sub-share sent privately as well as the `missing share' case where the share is encrypted with the public key and shared over Ethereum. 
\item Filed an \emph{unjustified complaint}, which is a complaint against a participant who followed the protocol precisely, i.e., did not perform any of the misconducts listed above. 
\item Did not file a complaint after detecting one of the misconducts $1-6$.
\end{enumerate}
\end{definition}

\begin{definition} [Successful run of DKG*]
A successful run of DKG* is one in which no complaints have been filed (excluding pings).
\end{definition}

\begin{claim}
In a successful run of DKG* properties C1, C2, C3 and S are met.  
\end{claim}

\begin{claim} [Liveness] 
If a run of DKG* was not successful, then one faulty participant has been detected and slashed.
\end{claim}

\red{this is more of a claim not a property}
\begin{definition} [\textbf{Liveness Property (L)}] 
Each run of the protocol is either successful \red{we should define this maybe more clearly...}, or else the deposit of \red{at least} one participant who did not follow the protocol \red{we defined `faulty', why not use it?} is slashed.
\end{definition}

\begin{remark} \label{RationalComplaints}
\red{David: Don't agree with everything here. Items 3-6 are related to data which is sent by $i$ personally to another participant $j$. This means that not any participant of the protocol can complain on this data, but only $j$. \name incentivizes participants to file justified complaints by rewarding them $1/2$ of the deposit of the faulty party. We thus assume that if $j$ does not complain in such a case, then $j$ is colluding with $i$, and therefore the data sent from $i$ to $j$ is irrelevant as they are in this context the same entity. In particular, we assume for the clarity of the analysis that if two nodes are colluding, then the data they send each other is consistent and compliant with the protocol.}
\end{remark}


\red{An examination of the protocol shows that the above list exhausts all the possibilities of an incorrect behavior. Note that each of the complaints listed above relates to one specific misconduct. We divide the misconducts to three: misconduct $1$ is ``un-rulable'' when the communication is off-chain and ``rulable'' when communication is on-chain. Indeed, in case $comp^1$ is filed, ``full'' DKG* \red{moves} to on-chain modes. Misconducts $2-7$ are detectable (note that misconduct $7$ is ``self-detectable'' as no node needs to file a complaint for it). Misconduct $8$ is the only non-detectable misconduct. To prevent nodes from failing to complain we must have the reward for complaining competitive with what the adversary might offer. This is in high view how we design our incentive structure.}   

An examination of the protocol shows that the above list exhausts all the possibilities of an incorrect behavior. To each faulty behavior we attach a \emph{complaint type} which corresponds to the specific subject of the complaint.

The last complaint $copm^6_{j,i}$ is filed whenever the subshare is inconsistent with the commitments - either with the set $X^1_{i,k}$ or with $X^2_{i,k}$. Respectively, checking this complaint requires computations in $G_1$, or in $G_2$. \red{However, since it is extremely expensive to make $G_2$ calculations over Ethereum}, we use wish to avoid these whenever we can. The following lemma enables us to avoid $G_2$ calculations when verifying $copm^6_{j,i}$.

\begin{lemma} \label{X1iffX2}
In the case all shares $X^1_{i,k}$ ,$X^2_{i,k}$ are pairing consistent (in the sense $copm^5_{j,i}$), then a subshare $\bar{x}_{i,j}$ is consistent with $X^1_{i,k}$ iff it is consistent with $X^2_{i,k}$. 
\end{lemma}

\begin{proof}
By \ref{PairingCollision} we know that if a pair of commitments $X^1_{i,k_0}$ and $X^2_{i,k_0}$ is consistent, then $X^1_{i,k_0}$ and $X^2_{i,k_0}$ are drawn from the same exponent $a_{i,k_0}\in Z_q$, namely that $X^u_{i,k_0}=g_u^{a_{i,k_0}}$ for both $u\in \{1,2\}$. We thus know that the commitments $X^u_{i,k}$ are drawn from a polynomial $\bar{f}_i:=\sum_{k=0}^t a_{i,k}z^k$. 


\red{Maybe replace the following paragraph with 'By simple basic group theory and polynomial arithmetic, we know that the unique exponent $x_u$ satisfying $g_u^{x_u}=\prod_{k=0}^t \big(g_1^{a_{i_k}}\big)^{j^k}$ is $\bar{f}_i(j)$. Thus  
$\bar{x}_{i,j}$ satisfies the above equation for $u=1$ iff it satisfies it for $u=2$, as wanted.}

given an element $g_u'\in G_u$, there is a unique exponent $x_u'\in Z_q$ such that $g_1^{x_u'}=g_u'$. In particular, let $x_u'\in Z_q$ be the exponent corresponding $g_u'=\prod_{k=0}^t \big(X^1_{i_k}\big)^{j^k}=\prod_{k=0}^t \big(g_1^{a_{i_k}}\big)^{j^k}$. As the simple polynomial arithmetic underlying this equation, we know that for both $u\in \{1,2\}$, $x_u'=\bar{f}_i(j)$, and in particular $x_1'=x_2'$. Now, if $\bar{x}_{i,j}$ satisfies the equation $g_1^{\bar{x}_{i,j}}=\prod_{k=0}^t \big(X^1_{i_k}\big)^{j^k}$, then $g_2^{\bar{x}_{i,j}}=\prod_{k=0}^t \big(X^2_{i_k}\big)^{j^k}$, and vice versa, as wanted. 

\end{proof}


The liveness property is now a direct result of the following two lemmas.
\begin{lemma} \label{ComplaintDetection}
Any of the faulty behaviors listed in \ref{FaultyList} is met with a complaint to the smart contract. 
\end{lemma}
\begin{proof}
\red{A successful complaint grants the issuer with at least $X/2$ Ether. By our assumption on rational participants (see \ref{RationalComplaints} above)}, we know that upon detecting a faulty behavior, a participant files a complaint to the smart contract with the specification of the faulty behavior. This reduces the proof to showing that any behavior from the list is detectable by at least one participant. Item $1$ is detectable not only by the participants of the DKG*, but by any entity with access to the Ethereum blockchain. Recall that although private and some of the public communication is done over \red{personal side channels}, not sending the data on time would reflect on the Ethereum ledger (\red{see handling not receiving data description above}, so also these scenarios are detectable by all. 

Items $2-3$ are detectable as all three relevant groups $G_1,G_2$ and $\Gamma$ admit an efficient algorithm for checking group membership. Verifying the set of commitments match the Merkle root published on Ethereum is done by computing locally the Merkle root of the commitments and comparing the value with the public one. Item $5$ is simply checking $t+1$ pairings, and item $6$ is simply checking an equality in elliptic curve groups. Both these are efficiently computable, which concludes the proof.

\red{what about item $4$? And we probably need to say something about items $7-8$. Also, note that this discussion relates to the discussion above after remark 14 that starts with "An examination of..."}
\end{proof}

\begin{lemma} \label{SlashingLemma}
Any complaint filed to the smart contract by $j$ against $i$ results in the slashing of exactly one participant: $i$ in case of a justified complaint, and $j$ otherwise. 
\end{lemma}
\begin{proof}
The proof should establish tow facts. First, that for every complaint there exists an algorithm which uses only the data available to the smart contract and unambiguously determines if the complaint is justified or not. Second, that the smart contract can execute this algorithm, in particular that it is within the computational capabilities of the contract. While the first part is concerned with the design of DKG*, the second has more to do with the computational limitations of Ethereum. The proof proceeds by inspecting each complaint and specifying the algorithm for verifying this complaint. We also explain why the smart contract has the required data for the algorithm to work. Finally, we summarize the computational requirements from the smart contract to execute each such algorithm. The summary is given in a table below, and concludes the proof.

\red{Consider adding a pseudo-code of the smart contract and reference the relevant functions.}
\begin{enumerate}
\item $copm^1_{j,i}$ By definition, the complaint is justified iff the required data was not published and the phase timeout has passed. It is thus straightforward to verify whether this complaint is justified or not. There is virtually no computation needed to be done---the smart contract keeps a variable for each participant, whether she published the necessary data or not.
\item $copm^2_{j,i}$ Checking group membership is done by raising the element to the power of the group order and verifying the result equals the identity element of the group. The group order is hard coded in the smart contract and the public key for encryption may be found in $i$'s enrollment transaction.
\item $copm^3_{j,i}$ By the same reasoning as above, given $X^u_{i,k_0}$ there is an easy way to check group membership. Moreover, since the complaint contains an Ethereum transaction signed by $i$ containing the set of commitments, the smart contract may verify that this set of commitments was indeed sent by $i$. It can thus determine whether $X^u_{i,k_0}$ is indeed in $G_u$ or not. 
\item $copm^4_{j,i}$ Checking this complaint amounts to calculating the Merkle root (resp. Hash value) of the set of commitments (resp. of $X^u_{i,0}$). As with the previous complaint, the set of commitments is included in the complaint in an authenticated way. So the smart contract can make this calculation. Since we assume $H$ is \red{second} pre-image resistant, this check unambiguously determines if $i$ was faulty or not. \red{we need to relate to pre-compiled contracts for the hash computation here also. We can also say that there could be optimizations made here.}
\item $copm^5_{j,i}$ Checking the validity of the complaint amounts to calculating two pairings, for which there is an efficient algorithm. Specifically, the pairing we use may be calculated using a designated pre-compiled contract \red{(see above)}. Once again, the authenticated set of commitments is included in the complaint. Since $X^1_{i,k_0}, X^2_{i,k_0}$ are included in the complaint, and $g_1,g_2$ are hard coded into the smart contract, all of the required data is available to the smart contract.
\item $copm^6_{j,i}$ From lemma \ref{X1iffX2}, it is enough to check consistency of $\bar{x}_{i,j}$ with $X^1_{i,k}$. Given all the commitments $X^1_{i,k}$ and the sub-share, checking this amounts to performing several $G_1$ operations. The commitments are once again included in the complaint in an authenticated way. The sub-share is also included, in one of two ways: either it was sent privately to $j$ as is done in a 'happy flow' scenario, or else the sub-share was encrypted using $j$'s public encryption key and uploaded by $i$ to the smart contract. In the former case, $j$ includes the sub-share sent to her by $i$, in an authenticated way, similar to the commitments, thus making it known to the smart contract. In the latter, $j$ includes $\xi_j$, allowing the smart contract to decrypt $i$'s transaction which included the encrypted sub-share. Either way, the smart contract can now perform all required group calculations and rule the complaint justified or not. \red{Missing gas estimations.}
\end{enumerate}
\end{proof}

By definition of QUAL in \cite{DKGRevisited}, any participant in QUAL has successfully completed a Feldman secret sharing. Recall this means each participant shared a set of polynomial sub-shares $\bar{x}_{ij}$ and public commitments which are consistent with those sub-shares. 
\begin{lemma} \label{QUALisALL}
A successful run of DKG* with participants $\{1,\dots,n\}$ is an implementation of a joint-Feldman protocol \red{(is this defined anywhere? Is this related to the Joint-Feldman lemma in section 4.3?)} resulting in $\text{QUAL}=\{1,\dots n\}$.
\end{lemma}
\begin{proof}
\red{I think this can be explained better.}
By definition, a successful run is a run which ended with no complaints. In particular, by \ref{ComplaintDetection} above, this means all \red{correct} participants received the public commitments $X^2_{i,k}$ from \textbf{all} other participants, and that each participant $j$ received a share $\bar{x}_{i,j}$ which is consistent with these commitments. This proves the claim. 
\end{proof}

\red{I'd replace this by what I put above. Also, if this is the main result we want to show, it should be up top and all the lemmas and claims build towards the proof, which i believe can be much shorter.}
\begin{theorem}
DKG* admits the correctness properties (C1),(C2),(C3), the secrecy property (S), and the liveness property (L).
\end{theorem}
\begin{proof}
\noindent{\textbf{L}} This is a direct result of \ref{ComplaintDetection} and \ref{SlashingLemma}.

We continue by showing that each successful run of the protocol admits the correctness and secrecy properties.

\noindent{\textbf{(C1)}} By \ref{QUALisALL} we know that $QUAL=\{1,\dots,n\}$ and in particular that at the end of the run all participants hold the same set QUAL of no disqualified participants. From now on the proof proceeds exactly as in \cite{DKG}. \red{Maybe give the idea of the proof?} \red{Maybe add their proofs as an appendix? David: good idea}

\noindent{\textbf{(C2)}} In \name the values $g_1^x,g_2^x$ are determined deterministically already at the enrollment phase, where each of the participants commits to its own contribution $X^1_{i,0},X^2_{i,0}$ by publishing, over Ethereum, the values $H(X^1_{i,0})$ and $H(X^2_{i,0})$. If later, the values $X^1_{i,0},X^2_{i,0}$ are publicly sent to all participants, and the values $g_u^x=\prod_{i=1}^n g^{X^u_{i,0}}$ (for $u\in \{1,2\}$), may be calculated by any participant. If some $X^u_{i,0}$ is inconsistent with its hash commitment at enrollment, then by \ref{ComplaintDetection}, this is detected and the run is not successful. The fact that $x$ is indeed the same secret which is promised by (C1) is immediate by the definition of the Feldman secret sharing protocol. 

\noindent{\textbf{(C3)}} Once again, the value $x\ mod\ q$ is deterministically defined once the commitments $H(X^1_{i,0})$ and $H(X^2_{i,0})$ are published in the enrollment transaction, due to the bijection between $G$ and $Z_q$. And so, since $x=\sum_{i=1}^n a_{i,0}$, $x$ is uniformly distributed in $Z_q$ \red{so long as at least one participant $i$ sampled $a_{i,0}$ uniformly from $Z_q$, and so long as this participant did not publish any information about $a_{i,0}$ before the end of the enrollment phase}. 

\noindent{\textbf{S}} Since DKG* admits property (C3), the simulation argument given in \cite{FeldmanVSS} may be used to prove secrecy (see also the appendix of \cite{DKGRevisited} for a concise review of the argument). \red{The only thing that is different is that in our protocol we publish some more information, and we have to show a simulator can simulate that as well. David: seems like it's required then.}
\end{proof}

\red{There are three essential differences between our protocol and \cite{DKGRevisited}, namely the slashing mechanism which replaces the agreement on the set QUAL; the public key is the pair $(g_1^x,g_2^x)\in G_1\times G_2$ instead of $g_1^x\in G_1$ \red{$g_2^x\in G_1$} \red{(I don't think this is something to mention. David: well, we can say that this is an artifact resulting working over Ethereum, and is what enables the efficient computations over Ethereum.)}; and finally, our scheme doesn't assume an abstract communication layer, but suggests one in practice---Ethereum.}

\red{Also, I think the major differences are that our protocol doesn't necessarily but it restricts the strategy space of the corrupted actors. Also, in a sense, revealing $t$ ``sub-secrets'' may be problematic---while theoretically it reveals nothing on $f_i$, in practice it reduces $i$'s protection from $t+1$ secrets which she can hide in different places to only just one. This might be something to mention. Also, it would be nice to include a discussion on the economic adversary model and what happens if the  assumptions break---at most $t$ malicious actors or $t<n/2$.}

\red{David: What is this paragraph?}|
\red{Our liveness proof deals with the construction of QUAL, rendering not manipulable in a successful run. Publishing the pair $(g_1^x,g_2^x)$ is compliant with the framework of asymmetric pairings presented in \cite{AssymetricPairings}. (Ido: Maybe some work is needed here but I don't think so.). And finally, \ref{CommSecurity} shows that our private/public communication channels are indeed private/public (resp.). All other modifications of the proofs to our setting are rather straightforward. We begin with the liveness proof.}


%\paragraph{Sketches of Proofs} (C1) follows directly from the fact that any honest party can \textit{verify} during the protocol whether or not its share is indeed a valid share. A run of the protocol terminates successfully only if all shares of honest parties are valid. (C2) is dully obtained as the public key $(g_1^x,g_2^x)$ is published on the Ethereum blackboard. The fact that it corresponds to the secret $x$ follows by the same reasoning as above for (C1). (C3) is guaranteed as the commitments to the values $g_1^{a_{i0}},g_2^{a_{i0}}$ are hidden by first publishing only the hash values of $g_1^{a_{i0}},g_2^{a_{i0}}$. Secrecy is proved via a simulation argument: it is the same proof as in~\cite{DKG}. Liveness is easy by design.


%The security properties should be proven formally: If $H$ is a random oracle and $G$ is a GDH group bla bla... Really there is a lot here, except of the formal proofs. We need to work with divide-and-conquer. 



==> implementation.tex <==
\subsection{pairing computation gas consumption}
\subsection{transaction size, smart contract computation required.}



==> intro_new.tex <==
\paragraph{What are we solving:} making sure a secret is secret up to a certain point in time and reveled from a certain point in time (in rational environments). Setting economic constraints on this secrecy. \red{This is very concrete and one application we found, but in a more general tone, we define a new model in which threshold cryptosystems could not have existed until now and make the necessary modifications to make them fit the model. The model is different to the previous model in its economic nature and the rational nature of the participants.}

\paragraph{Other solutions:} Threshold cryptosystems (secret sharing), PoW, VDFs, low-influence functions.

\paragraph{Where do they fall short:} collusion pressure which turns the random generator useless.

\paragraph{Why interesting:} leader election for lottery or blockchain/consensus applications.


\red{In a sense we build a threshold cryptosystem as a second layer application over Ethereum.}

\red{To date, the natural (perhaps only) candidate that could facilitate such an escrow service is the Ethereum blockchain. However, Ethereum is (and should be regarded as) a scarce public resource that is to be used only when absolutely necessary. Ethereum resources: be it forward transactions to the entire network of miners and nodes, process transactions and invoke redundant computation, or have data written to the blockchain, replicated thousands of times.}

Threshold cryptosystems require an initial key distribution step. A well-known approach to DKG for threshold cryptosystems is the Ped-DKG protocol (or Joint-Feldman) which relies on Shamir secret sharing. We rely on Ped-DKg and adjust it for an economic model. Our contributions in this paper are:
From a purely cryptographic perspective, we add hash commitments to handle the malleability problem identified in~\cite{} and check group membership of the commitments which is usually omitted although seems necessary for the proof. On top of the original DKG protocol, we build an incentive layer that depends on a trusted escrow that holds the participants' deposits. This allows two main capabilities: First, every complaint submitted fails the protocol and invokes slashing. Second, after the DKG and during the time the cryptosystem itself is being used, a framing mechanism is introduced. The main motivation behind framing is to \red{discourage/dismantle} the collusion pressure that is inherent to many threshold cryptosystems. Most significantly, the framing mechanism allows us to consider an economic model, where value is produced by the cryptosystem and should be handled according to some predetermined notion of fairness (set by the designer of the system). While this might seem a bit obscure, we give a motivating example.  

\red{We adapt a specific distributed protocol to use Ethereum as an arbitration entity and demonstrate how the distributed protocol itself can be simplified and enhanced by economic incentives. This serves a great case-study for general purpose layer two solutions that are being currently designed and studied.}

\red{Second layer interpretation: this is very similar to any second layer protocol. We define a set of complaints (which Ethereum can efficiently arbitrate) and prove they are enough to ensure our threshold cryptosystem satisfies the desired (economic) properties\footnote{\red{In our Bitcoin analogy this is like having a very clear estimation of how much would it cost to get 51\% of the hash power, and having mechanisms that reduce the profitability of collusion.}}.}


==> introduction.tex <==
\underline{From the DKG side:} Recently, a new approach to realize randomness beacons, based on unique digital signatures has gained much interest in the blockchain space (\cite{Algorand}, \cite{Dfinity}). BLS signatures are a good candidate for such signatures. Indeed, in~\cite{Dfinity} threshold signatures are used as part of the ``threshold relay service'', a service that periodically emits random values. It is desired that these values are (i) unpredictable and (ii) non-manipulable. In case the $t$ assumption breaks any DKG protocol would leak the scheme's secret breaking requirement (i). However, in typical DKG protocols (\cite{GJKR}, \cite{PedersenDKG}) if this assumption breaks, the secret key can be chosen to the liking of the corrupted participants, yielding in their potential control over the emitted values for a long period of time. We improve on these protocols in the case the $t$ assumption breaks, reassuring the secret key is not controllable by the corrupted nodes (but only revealed).
Also, we need less communication assumptions or assumptions regarding active participation. We can motivate correct participation, be it publish consistent data, verify data others publish, or file complaints when they are detected.
Also, setup is taken care of via enrollment to a smart contract.

We define the concept of ``economic adversary'', instead of just assuming a rather arbitrary bound on the number of corrupted nodes. This is in the spirit of ``economic finality'', an idea from Casper FFG~\cite{}.

\underline{From the Ethereum side:} We show a specific second layer dapp that can actually be helpful. We also show that efficient elliptic curve operations can be useful for realizing different cryptosystems over Ethereum. In this case pre-compiled contracts for SNARK verification is used to realize a DKG protocol for a BLS-3 threshold signature scheme.
Ethereum is interpreted as a reliable public one-phase broadcast channel.

\paragraph{In the context of randomness beacons}
RANDAO requires all participants to sign---this generates great difficulties as in practice participants might have temporary disconnections and they should not be significantly punished for it (this would discourage participation) and the liveness of the protocol becomes too vulnerable---including, bribing only one entity could put the protocol to a halt.
\red{We should have $t>n/2$ so that if more than one $t+1$-coalition emerges, there will be some overlap between them.}  

%Some computations may result in complaints being filed to the smart contract. In our protocol, as opposed to the GJKR DKG~\cite{}, every complaint results in aborting the protocol and slashing the deposit of a \red{faulty} participant. In particular the smart contract performs computations and unambiguously decides which participant was \red{faulty} (and thus caused the abortion of the protocol). 
    

==> protocol.tex <==
As the designers of a threshold cryptosystem we have a clear notion of how it should evolve and how should the participants behave. It is of our duty to build the incentives such that indeed the participants act as expected and do not have some clever way to act unexpectedly and gain unfair profit. 



Eth-DKG adapts the \red{Ped-DKG} protocol described above, to benefit from a public blockchain infrastructure---the Ethereum blockchain. Ethereum is used for two main purposes. First, we use it as a censorship-resistant and publicly available broadcast channel. Second, it serves as a trusted escrow service that collects and redistributes deposits according to a predetermined set of rules. This escrow service serves as a crypto-economic layer which significantly reduces the colluding pressure inherent to threshold cryptosystems and simplifies the protocol.

The section is organized as follows. We begin by describing our model assumptions, \red{(highlighting the economic nature of our adversary)}. We then extend the set of requirements in Sec.~\ref{properties} with a critical \red{\emph{incentive compatibility}} requirement. Next, we specify the design choices we were forced to make in order to be able to use Ethereum as an arbitrator that has to verify costly elliptic curve computations. Finally, we describe Eth-DKG as a client-smart contract system. We start off with a \red{``light''} version that is fully contained within Ethereum, but is rather expensive and applicable only when $n$ is small \red{($\approx 50$)}. The \red{``full''} version, presented afterwards, reduces on-chain usage and scales with $n$ \red{($\approx 1000$)}.
%We describe the phases of the protocol and give a detailed description of the transactions it uses. At first we give a 'happy flow' run of the protocol, omitting the explanation of how complaints are handled and merely specifying exactly when and why complaints are filed. We then conclude the description and give a detailed explanation of how each complaint is dealt with.

\subsection{Model}
\red{Our main effort in defining an economic adversary is to eliminate the colluding pressure inherent to the protocol. For this, we first define the minimal notion of ``colluding''---sharing secret information that could not have been discovered honestly (e.g., $P_i$ sharing with $P_j$ the values $f(i)$ or $f_i(k)$ for some $k\neq j$). The core insight is that once such an exchange of secret information took place, $P_j$ can frame $P_i$ unambiguously. We build the economic structure such that the risk of being framed reduces the colluding pressure. Essentially, the first secret exchange of information would lead a rational participant to frame her partner as we assume she prefers the reward over the successful termination of the protocol (or the extra information she gains from the collusion). Note that in the case of sharing $f_i(k)$ it is not clear who shared the secret---$k$ or $i$. In this case, both players would be slashed, but the fear of anyone of them of being slashed should discourage anyone of them from sharing the information. Also, the rewards should be split in a way that does not allow the collusion of say $j$ and $k$ against $i$. To conclude, the unambiguity would never include three players.}

Our model resembles the original model presented above. We enhance the model with a trusted execution environment that can take deposits and slash misbehaving participants according to some predetermined logic. Particularly, we assume each player runs an Ethereum full node and has an Ethereum wallet with some Ether balance. Regarding communication, we assume that the participants are connected by a mesh network of private channels. We do not restrict this network to be synchronous. For public broadcast we use Ethereum which we view as a synchronous communication channel.

\subsection*{Economic collusion pressure}
The need to consider an adversary in the context of a DKG protocol lies in the understanding that the produced key shares hold value. %which is derived from the power they \red{proffer/demonstrate} within the cryptosystem they enable. 
Moreover, the more key shares a participant has, the more power she holds within the cryptosystem, where $t+1$ key shares give her complete control. This motivates entities to get hold of as many key shares as possible and introduces \emph{collusion pressure}. Since modeling this pressure is complicated, the classic way to handle it is to assume a limited adversary that can corrupt (and coordinate) at most $t$ of the participants. In essence, the notion of the adversary obfuscates the interests of the participants and puts a bound on the ``degree of collusion'' possible in the system. In particular, assuming this bound is $t$ in the DKG scenario is rather ironic---an adversary controlling $t$ players is unlikely to stop there as she is highly motivated to corrupt the $t+1$ player and get control of the underlying cryptosystem. 

For these reasons, we take a different approach and consider the participants as rational entities that act selfishly and aim to maximize a profit. To this end, they wish to get hold of as many key shares as possible (on top of their valid one). \red{However, they would rather take an immediate profit of $D/2$ Eth than obtain one more key share. We assume the typical way to get hold of key shares is by trading or exchanging them. Finally, we assume players refuse to lose more than $D$ Eth and that the total profit from gaining total control of the cryptosystem (that is, getting hold of $t+1$ key shares) is valued less than $t\cdot D$. Note that estimating $D$ is still a complicated task that depends on the underlying cryptosystem and its value proposition.}

This set of assumptions is very simple and captures two important notions. First, demand for key shares is inevitable and thus a market price for them would evolve (under our setting we assume this price would be kept below $D/2$). Second, the players as driven according to the strategy that maximizes their profits---they have a basic motivation to have a functioning threshold cryptosystem (because it results in a profit), but an immediate profit of $D/2$ is more beneficial for them.

Our terminology is quite different---instead of talking about the adversary corrupting players, we talk about players colluding with one another to pursue their interests. To make this formal we define the basic concept of collusion between two players.

\begin{definition} [Collusion]
Players $P_i$ and $P_j$ are said to have colluded if $P_i$ has shared a secret with $P_j$ which could not have been found by $P_j$ using the information she received rightfully during the protocol (or vice versa).  
\end{definition}

%We assume a similar adversary---static that can corrupt at most $c$ participants. We set $t$ (the degree of the polynomial) to be $\max\{ c,n-c \}$, eliminating the ability of the corrupted participants to get control of the cryptosystem or \red{put it to a halt}. check the $t<n/2$ assumption.

\subsection{Eth-DKG design rationale}
We have two main design guidelines: building an \textbf{incentive compatible protocol}, which is \textbf{cheap and scalable} (in the sense of the number of players $n$). 

In high level Eth-DKG is very similar to the protocol in Fig.~\ref{}. However, the use of Ethereum allows extra capabilities. First, in order to participate a deposit of $D$ Eth would have to be made. Then, during the run of the protocol, if a misconduct (we give an exhaustive list of all possible misconducts) is detected, a player is incentivized to file a complaint as she would get rewarded if the complaint is found just (by Ethereum). In the same spirit, players would avoid misbehaving as they fear being complained against, losing their deposit. This type of complaint mechanism covers all detectable misconducts. However, collusion (as defined formally above) is undetectable and thus the risk of coalitions exists. To eliminate this risk we introduce an additional mechanism---framing. Framing amounts to publishing information that could not have been obtained other then by collusion. When framing is possible, participants are afraid to collude as any (meaningful) collusion leaves traces that could be used for framing. Moreover, players that can frame are incentivized to do so for the anticipated reward.

Second, since compensation is possible, failing the protocol becomes a viable option. Eth-DKG enforces a complaint mechanism that rewards valid complaints thus letting us assume participants that detect misbehavior would indeed complain. Moreover, since we design the protocol in a way that any misconduct is detectable (apart from not complaining), we can deduce that no player would misbehave (from fear of being slashed).

%there are two types of undetectable misconducts---collusion and not complaining 

Failing the protocol while slashing one's deposit enables us to simplify the protocol by having the first complaint filed fail the protocol. This of course relies on a trusted environment to escrow the deposits, and arbitrate disputes.

The one complaint logic achieves two things: the best strategy of any \red{player/coalition} is to follow the protocol, as otherwise they would lose their deposit. Additionally, sub-shares are never revealed in public as part of the protocol. Another unprobable strategy is that of ``not complaining'' as it implies a loss. Finally, our incentive structure and the framing mechanics makes the formation of coalitions extremely unprofitable.

This might be thought of as a caveat of our system---a single dispute may terminate the execution of the protocol, failing the generation and distribution of keys. While this seems like a disadvantage, we show that any correct participant that follows the protocol's instructions, leaves the protocol ``happy''. That is, either the protocol ended successfully, in which case, she and the entire set of participants have keys for a functioning $(t,n)$-threshold cryptosystem, as intended. Or, she is compensated by a sum she values higher than her participation in the threshold cryptosystem. Additionally, she can now restart the DKG protocol from scratch.

Recall the GJKR protocol also utilizes a complaint mechanism to determine the set QUAL. There, a zero-tolerance dispute mechanism is impossible as any single participant may have been corrupted by the adversary. Only $t+1$ participants advocating the same claim can be trusted. The zero-tolerance philosophy introduces a difficulty though---making sure that if indeed the protocol fails, an adequate compensation has been distributed among the correct participants. We refer to this as an ``incentive compatibility'' requirement which we formulate and prove in Sec.~\ref{}.   

\red{These are translated to a few principles:  
We allow the protocol to fail in return for a proper compensation for each correct participant.
We refuse to reveal sub-shares in public as part of the protocol.
We set as a goal to restrict the range of possible malicious strategies to minimum.
Avoid using an expensive public resource, Ethereum. 
We have a complaint mechanism, where the arbitrator is Ethereum and the complaints are unambiguously ``rulable'' (``un-rulable'' complaints (pings) are also possible but invoke more expensive ``rulable'' complaints). The first complaint would fail the protocol, slashing one \emph{faulty} (we define this formally) player's deposit and distribute it among the others.}    

\red{Adversary's goals:
fail the protocol without cost, know secret information, control the secret key, make correct nodes' keys useless.}

\subsection{Ethereum-specific concerns}
\red{We should emphasize here the limitation dictated by the pre-compiled contracts and the fact only a very restricted set of operations can be done efficiently over Ethereum.}

At this point the reader understands the motivation to implement DKG over Ethereum---reducing colluding pressure under economic adversary. However, working over Ethereum and having it serves as an arbitrator comes at a cost. Ethereum is an expensive and limited ``global computer''---general elliptic curve computations (which are necessary for handling complaints) would be unfeasible to execute, and writing the protocol's data on the Ethereum blockchain (when $n$ is rather large) would be practically unfeasible. To handle these constraints, we take advantage of specific pre-compiled contracts (addition, exponentiation and pairing in specific elliptic curve groups) that have been incorporated into the EVM in the Byznatium hard-fork \red{(verify this and add citations and names of the pre-compiled contracts)}\footnote{It is interesting to note that these pre-compiled contracts have been developed for SNARK verification and we were able to use them for our DKG.}. However, this restriction somewhat complicates the protocol and adds an unnatural step. To reduce the amount of data written to Ethereum we use common commitment techniques.

We note that the keys obtained by the Eth-DKG protocol correspond to a BLS-3 threshold signature scheme that is assumed to be secure but is more recent than other signature schemes and relies on an additional cryptographic assumption (co-DHP*, see background). We shall emphasize that the restriction to a specific cryptosystem originates from the current state of Ethereum. In general, our protocol is agnostic to the underlying groups and cryptosystem. If Ethereum or another public blockchain would enable elliptic curve computations in other curves, the protocol could be used for other cryptosystems.

Having understood the limitations imposed by Ethereum and even after opting to adjust to its constraints, Ethereum remains a scarce public resource which is expensive to use. We thus design Eth-DKG to have minimal interaction with Ethereum, be it forward transactions to the entire network of miners and nodes, process transactions and invoke redundant computation, or have data written to the blockchain, replicated thousands of times. We use the Ethereum network only once disputes arise and as a final arbitrator.

\subsection{System parameters}
Before giving the full details, we give the general parameters of the system. All the participants must be aware of these parameters. The system parameters can be made public via the smart contract that is part of the system (or other channels): 
\begin{enumerate}
\item Number of participants $n$ and the threshold $t$.
\item $q,g_1,g_2,G_1,G_2$, where $G_1=\langle g_1 \rangle$ and $G_2=\langle g_2 \rangle$ are the cyclic (elliptic curve) groups of prime order $q$ described in the Ethereum Yellow Paper (\cite{ethereum}, see App. E.1). Note we are restricted to these groups---we were forced to build a scheme that works within these groups so that Ethereum may be useful. 
\item Description of the pairing $e:G_1\times G_2\rightarrow G_T$ also given in~\cite{ethereum}, App. E.1.
\item $D$, the sum (in Eth) participants should deposit.    
%\item $r,\gamma,\Gamma$, where $\langle \gamma \rangle=\Gamma$ is the cyclic group of prime order $r$ used for encrypting messages. \red{We need to choose one---I think we chose $G_1$. IDO: you cannot choose $G_1$, you don't mix these kind of things.}
\item A description of a hash function $H$ (Ethereum friendly).
\end{enumerate}


\subsection{Protocol Description}
\subsubsection*{General Settings/Basics}
The protocol is run by a client software that interacts with a smart contract over Ethereum. Every participant needs the client-side program and an Ethereum full-node running on its machine. Players \emph{enroll} to the protocol with their Ethereum address, and their Ethereum signature serves as a means to authenticate protocol messages.

Eth-DKG proceeds in phases, which roughly correspond to the phases of Fig.~\ref{FigGJKR}. Each phase begins as soon as the previous one ends and lasts at most $\delta$ Ethereum blocks \red{refer to the discussion on epochs above}. During each phase, the participants are typically asked to perform some computation and share information. They are asked to complain when they detect another player does not follow the protocol. In case of a complaint, the smart contract rules whether it is justified or not, slashing the faulty player accordingly and terminates the protocol. 

If no complaints are filed, the protocol results in a public key $(g_1^x,g_2^x)\in G_1\times G_2$, where $x$ is the secret key (known to no one), as well as with each participant holding privately a share $x_i$ for the secret key $x$. In addition, each participant holds the public key shares $(g_1^{x_j},g_2^{x_j})$ of all other participants, as well as public data which allows verification of the corresponding private key shares.


\subsubsection*{Two Variants} 
We describe two variants of Eth-DKG---on-chain and off-chain. In \red{Eth-complete}, all communication is done over Ethereum. It is thus more expensive in terms of gas and is restricted in $n$, but enjoys the property that it is completely contained within the Ethereum framework. \red{Eth-efficient} utilizes off-chain channels to reduce the interaction with Ethereum to minimum, and writes to Ethereum only data which is necessary for ruling complaints---mainly commitments to the data which is sent off-chain. It thus scales much better with $n$. On the other hand, it requires the players to independently establish peer-to-peer communication network. It also introduces the difficulty of handling complaints which involve private communication channels \red{see remark on consensus / broadcast channels)}. To this end we use \red{PING complaints}, which essentially drive the protocol to ``fall back'' to the Eth-complete variant, as explained below.

Fig~\ref{FigureEth-DKG} gives a detailed description of the protocol without explaining how complaints are dealt with, but only states when complaints should be filed. We elaborate on the complaint mechanism in \red{ref} below.

\red{Move this to the communication / Ethereum background.}
\underline{Epochs.} 
It is necessary for the correctness of the protocol to make it clear when phases begin and end. To this purpose we set each phase to last \textit{epoch} blocks, where the counting starts on the initial transaction deploying the smart contract, and each phase succeeds the previous one. \red{As Ethereum is an asynchronous network}, we need to define \textit{epoch} to be large enough so as to allow all participants enough time to read and write their data to the blockchain. We think of $epoch\approx 100$ blocks, having in mind scenarios such as network high-loads and DDoS attacks. 



%\begin{figure}  {
%{\centering\fbox{
%\begin{minipage}{45em}



\begin{mdframed}
\begin{enumerate}
\item[0] Deployment. The protocol formally begins when the smart contract is deployed. Any Ethereum account can deploy the contract.

\item[1] Enrollment. The relevant Ethereum accounts enroll to the protocol by submitting \emph{enrollment} transactions\footnote{These would typically be hard-coded into the contract, where each account is publicly known to belong to some ``real-life'' entity.}. We refer to the participants by their enrollment order $1\leq i \leq n$. To enroll, participant $i$ locally generates:
\begin{enumerate}
\item A random polynomial of degree $t$ over $Z_q$, $$f_i(z)=a_{i,0}+a_{i,1}z+\dots+a_{i,t}z^t$$

\item A private key for private communication over Ethereum, $\xi_i\in Z_q$

\item Commitments to $f_i$'s coefficients, $X^u_{i,k}=g_u^{a_{i,k}}$
for $u \in \{ 1,2 \}$ and $k \in \{ 0,\dots, t \}$
\end{enumerate}

She then submits her enrollment transaction 
$$tx_1(i)=\Big[ D,g_1^{\xi_i}, \Big(H(X^1_{i,0}), H(X^2_{i,0})\Big) \Big]$$
where:
\begin{enumerate}
\item $D$ is her deposit in Eth
\item $g_1^{\xi_i}$ is her public key for \red{ElGamal encryption}
\item $H(X^1_{i,0}), H(X^2_{i,0})$ are her hash commitments
\end{enumerate}

The phase terminates once $n$ addresses enrolled\footnote{In case less than $n$ addresses enrolled and $epoch$ blocks have passed, any Ethereum account may submit a \textit{revoke} transaction, aborting the protocol and returning the deposits.}.  

\item[2] Commitments. Every participant submits a \emph{commitments} transaction. For $i$, $$tx_2(i)=\big[\{ X^1_{i,k} \}_{k=0}^t, \{ X^2_{i,k} \}_{k=0}^t \big]$$

If a participant fails to submit her commitments transaction in time, anyone can file a \red{complaint} against her. 
            
\item[3] Commitments Verification. Every participant locally verifies the commitments of the other participants. That is, checking that for all $1\leq i\leq n$ and $0\leq k\leq t$ it holds that  
\begin{equation*}
\label{pairingCommitments}
e\big(g_1,X^2_{i,k}\big)=e\big(X^1_{i,k},g_2\big)
\end{equation*}

In particular, group membership of the commitments is verified. 

If some equality does not hold, anyone can file a \emph{pairing} complaint.
            
\item[4] Sub-shares. Every participant $i$ locally computes her sub-shares $x_{i,j}:=f_i(j)$ for all $j$, and for $j \neq i$ encrypts it using $j$'s public key and submits a corresponding \emph{sub-share} transaction 
$$tx_3(i,j)=\Big[ ENC \big( x_{i,j}, g_1^{\xi_j} \big) \Big]$$

If a participant fails to submit one of her sub-share transactions in time, anyone can file a \red{complaint} against her. 
            
\item[5] Sub-shares Verification. Every participant locally verifies the sub-shares destined to her are consistent with the public commitment. That is, participant $j$ checks that for all $i$ it holds that
\begin{equation*}
g_1^{x_{i,j}}=\prod_{k=0}^t \big(X^1_{i,k}\big)^{j^k}
\end{equation*}
%\begin{equation}
%\label{shareVerification2}
%g_2^{x_{i,j}}=\prod_{k=0}^t \big(X^2_{i,k}\big)^{j^k}
%\end{equation}

If some equality does not hold, $j$ files a \textit{sub-share} complaint.
            
\item[6] Secret key share. Every participant locally computes her final secret key share. For $i$, $x_i:=\sum_j x_{j,i}=\sum_j f_j(i)=f(i)$.

\item[7] Public key. \red{To complete the DKG, the smart contract should be aware of the scheme's public key.} Any participant can send a \emph{public key} transaction $$tx_4=[(X^1_0,X^2_0)]$$ where, $X^u_0:=\prod_i X^u_{i,0}=\prod_i g_u^{f(0)}$. 

\item[8] Public key verification. Every participant verifies locally the submitted public key. If an invalid $tx_4$ was submitted, any participant can file a complaint---either a \emph{public key pairing} complaint or a \emph{public key $G_1$} complaint. If no $tx_4$ was submitted, the protocol fails with all deposits burnt. 

If no complaint was filed during phase $8$, the DKG protocol \emph{terminates successfully}. Note that the deposits are kept until the termination of the underlying cryptosystem.
\end{enumerate}
\end{mdframed}
%\caption{Eth-complete}
%\end{minipage}}}
%\par}\end{figure} \label{FigureEth-DKG}



% \underline{Eth-DKG---Variant 1}
% The protocol advances in fixed-length phases that last for $epoch$ blocks. We describe the phases. 
% \begin{enumerate}
% \item[\textit{Phase 0}] Deployment. Any Ethereum address can send a deployment transaction $Tx_0$ to deploy the smart contract.
% We denote the block number of this transaction by $B_0$.




% \item[\textit{Phase 1}] Enrollment. Any Ethereum address $i$ wishing to participate, performs the following computations privately:

% \begin{itemize}
% \item[-] Generates a random polynomial over $Z_q$ of degree $t$ $$f_i(z)= a_{i,0} +a_{i,1}z+\dots +a_{i,t}z^t$$

% \item[-] Computes $X^1_{i,k}:=g_1^{a_{i,k}}$ and $X^2_{i,k}:=g_2^{a_{i,k}}$.

% \item[-] Generates random numbers $\xi_{i,j}\in Z_r$ for $1\leq j\leq n$ and $j\ne i$. These would serve for a DH key exchange with all other participant to communicate private data. \red{what are we going for? the static or regular? I think the static would be much simpler to present.} 
% \end{itemize}

% sends an enrollment transaction to the smart contract, containing:

% \begin{itemize}
% \item[-] A deposit of $D$ ether to the smart contract 
% \item[-] A public key $\gamma^{\xi_i}$ \red{(I think this can be $g_1^{\xi_i}$)}
% \item[-] $H\big(X^1_{i,0}\big), H\big(X^2_{i,0}\big)$
% \end{itemize}

% From this point on, participants are asked to issue protocol transactions from the Ethereum address with which they enrolled. Other transactions are ignored. The participants are ordered according to their enrollment order and we denote them by their order $1,\dots, n$.            

% The phase terminates once $n$ addresses enrolled or \textit{epoch} blocks from $B_0$ have passed. If less than $n$ participants enrolled by this point, any Ethereum address may send a \textit{revoke} transaction, aborting the protocol while having the smart contract return the deposits. \red{footnote: we note that the appropriate way to construct the contract would be to have certain Ethereum addresses hard-coded into the contract, where these addresses are known to belong to the ``real-life'' entities that wish to engage in a DKG protocol.}

% \item[\textit{Phase 2}] Commitments. Each participant $i$ publishes commitments to its random polynomial by sending a transaction containing the data $X^1_{i,k}=g_1^{a_{i,k}}$ and $X^2_{i,k}=g_2^{a_{i,k}}$ for $0\leq k\leq t$. 
            
% \item[\textit{Phase 3}] Commitments Verification. Each participant privately verifies that for all $1\leq i\leq n$ and $0\leq k\leq t$ the following equalities hold:
% \begin{equation}
% \label{pairingCommitments}
% e\big(g_1,X^2_{i,k}\big)=e\big(X^1_{i,k},g_2\big)
% \end{equation}

% In particular, group membership is verified for each commitment. If an equality does not hold for some $i$ and $k$, then any participant may file a \textit{pairing commitment failure} complaint, including the pair $(i,k)$ for which the verification above failed. 
            
% \item[\textit{Phase 4}] Shares. Each participant $i$ computes privately the values $x_{i,j}:=f_i(j)$, and encrypts each of them using the encryption scheme explained in Sec.~\ref{DHXOR}, namely $e_{i,j}:=x_{i,j} \oplus  H\big(\gamma^{\xi_i\cdot \xi_j}\big)$. It then sends a transaction containing the data $\{e_{ij}\}_{j\ne i}$.
            
% \item[\textit{Phase 5}] Share Verification. Each participant $j$ privately verifies that the shares it received from another participant $i$ are compatible with the public commitments made by $i$, by checking that the following equalities hold: 
% \begin{equation}
% \label{shareVerification1}
% g_1^{x_{i,j}}=\prod_{k=0}^t \big(X^1_{i,k}\big)^{j^k}
% \end{equation}
% \begin{equation}
% \label{shareVerification2}
% g_2^{x_{i,j}}=\prod_{k=0}^t \big(X^2_{i,k}\big)^{j^k}
% \end{equation}

% If some equality does not hold, $j$ files a \textit{invalid share} complaint, sending a transaction specifying the identity $i$ and which of the equations \ref{shareVerification1}, \ref{shareVerification2} did not hold. \red{Only $G_1$ operations can be made in the smart contract} 
            
% \item[\textit{Phase 6}]
% Each participant $j$ computes privately its final share $x_j:=\sum_i x_{ij}=\sum_i f_i(j)=:f(j)$.

% \item[\textit{Phase 7}] 
% Any participant can send a transaction specifying the public key obtained by the protocol, namely $X^2_0:=\prod_i X^2_{i,0}=\prod_i g_2^{f(0)}$. \red{(not yet) This invokes the smart contract to return the deposits to all participants, and terminates the protocol.} In case a wrong value is uploaded in this transaction, any participant can file an \textit{invalid public key} complaint \red{(note that this complaint would have to go through $G_1$)}. 

% \end{enumerate}

% \underline{On \red{STATIC} private communication in DKG*} 
% \label{DHXOR}
% The scheme is based on the Diffie-Hellman key exchange, using the shared key as a \red{one time pad (definition/explanation needed)} to encrypt the message $m$, and proceeds as follows. Let $G=\langle g \rangle$ be a group of prime order $r$ in which the co-DHP is assumed to be hard. $G,g$ are  published as a system parameter at initialization. Every participant $i$ generates a random number $\xi_i\in Z_r$ and includes $g^{\xi_i}$ in its enrollment transaction. $g^{\xi_i}$ serves as $i$'s public key, and by the end of enrollment phase, all participants would have published their public keys on the Etheruem blackboard. Each pair of participants $(i,j)$ now share a common secret key $k_{i,j}:=g^{\xi_i\cdot \xi_j}$. When $i$ wishes to send a private message $m$ to $j$ it publishes $c:=m\oplus H(i,j,k_{i,j})$ to the smart contract ($\oplus$ denotes XOR).
    
% Notice that the shared secret $k_{i,j}$ is obtained by the regular Diffie-Hellman key exchange protocol, with a slight modification. In the regular Diffie-Hellman protocol, a user $i=1$ that wishes to generate $n-1$ secrets to (pairwise) share with $n$ different users, should generate $n-1$ corresponding random values $\{\xi_{i=1,k}\}_{2\leq k\leq n-1}$, one for each secret. Our scheme utilizes a variant of what is called \red{\textit{static-static}??} Diffie-Hellman (examples can be found in \cite{NISTKeyGenerationSchemes} section 6.3), in which a single random value is used multiple times. In our case this value is reused across different users \red{(at most ?? times)}. 
       
% \paragraph{\textit{Transactions.}} \red{Let's incorporate these into the protocol description, reducing words for succinct notations.} We describe the transactions used by the participants of the protocol, including their role in the protocol, the computation they invoke or that is required from the issuer of the transaction. See Table~\ref{TxSizeTable} for a summary of the contents, size and gas price of the transactions.
        
% \red{Notice that all transactions are trivially signed by their Ethereum address which serves as an authentication for the identity of the issuer.} 
% \begin{enumerate}
% \item{\textit{InitTx}} \red{Contains a code which deploys the smart contract.}
% \item{\textit{EnrolTx}} Enrollment transaction. For participant $i$, includes the following data: 
% \begin{enumerate}
% \item $D$ Ether deposit to the smart contract.
% \item $\gamma^{\xi_i}$ \red{$g_1^{\xi_i}$}, a public key for encrypting messages. 
% \item $H(X^1_{i0}), H(X^2_{i0})$.
% \end{enumerate}
                
% \item{\textit{CommTx}} Commitments transaction. For participant $i$, includes $i$'s commitments to the polynomial $f_i$: $X^1_{i,k}:=g_1^{a_{i,k}}$ and $X^2_{i,k}:=g_2^{a_{i,k}}$ for $0\leq k\leq t$.
            
% \item{\textit{SharesTx}} Shares transactions. For participant $i$, includes the shares $x_{ij}:=f_i(j)$, encrypted. Namely, $e_{ij}:=x_{ij} \oplus  H\big(\gamma^{\xi_i\cdot \xi_j}\big)$
             
% \end{enumerate}

% In addition to these transactions there is another class of \textit{complaint transactions}. According to the protocol, a complaint transaction is filed by any participant who detected an incorrect behavior of another participant. This can happen if, for example, participant $j$ computes and detects the commitments sent by node $i$ in the commitments transaction are inconsistent with the share $x_{i,j}$ $j$ received in the shares transaction. 
        
% Since many of the complaints are only relevant in the full version, we postpone the complete presentation of the complaints transactions to the end of this section (see Sec.~\ref{complaintsList}).
                
% \underline{DKG over Ethereum---Full Version}
% The essential difference between the simplified and full version of the protocol is in the communication aspect. To optimize the use of the Ethereum blockchain, we use standard techniques of hash commitments to minimize the interaction with Ethereum. In the spirit of a second layer solution, we relate to Ethereum as an extremely expensive resource whose use is to be reduced to the bare minimum. We leave the enrollment transaction and as fine-grained as possible complaint transactions that invoke minimal computation and data usage on the Ethereum blockchain. Note that for clarity and space, in the description below we leave many technical edge cases untouched. 

% \begin{itemize}
% \item[\textit{Phase 0}] Deployment. Any Ethereum address can deploy the smart contract by sending a deployment transaction. We denote the block number of the deployment as $B_0$. (Every participant needs the client-side program and an Ethereum full-node running on its machine.)

% \item[\textit{Phase 1}] Enrollment, from block $B_0+1$ to $B_0+epoch$. In a successful execution of DKG*, the enrollment phase is the one that invokes the most usage of Ethereum. Any Ethereum address $i$ wishing to participate, performs the following computations locally:

% \begin{itemize}
% \item[-] Generates a random polynomial over $Z_q$ of degree $t$ $$f_i(z)= a_{i,0} +a_{i,1}z+\dots +a_{i,t}z^t$$

% \item[-] Computes $X^1_{i,k}:=g_1^{a_{i,k}}$ and $X^2_{i,k}:=g_2^{a_{i,k}}$.

% \item[-] Generates a private and public key pair $\xi_i \in Z_r$ and computes $\gamma^{\xi_i}$.
% \end{itemize}

% she then sends an \emph{enrollment transaction} to the smart contract, containing:

% \begin{itemize}
% \item[-] A deposit of $D$ ether to the smart contract.
% \item[-] The public encryption key $\gamma^{\xi_i}$.
% \item[-] $H\big(X^1_{i,0}\big), H\big(X^2_{i,0}\big)$.
% \item[-] The Merkle root of the commitment Merkle tree, containing as leaves $X^1_{i,k}$ and $X^2_{i,k}$ for $k=0,\dots, t$.
% \end{itemize}           

% The phase terminates once $n$ addresses\footnote{Either pre-determined and explicitly indicated within the smart contract or arbitrary, depends on the setting.} enrolled or \textit{epoch} blocks from $B_0$ have passed. If less than $n$ participants enrolled by this point, any Ethereum address may send a \textit{revoke} transaction, aborting the protocol, having the smart contract return the deposits.

% From this point onwards, the participants have three types of system-identity: first, their Ethereum public-key with which they enrolled. Second, an index number $i\in{1,\dots,n-1}$ which is determined according to the order of the enrollment transactions in Ethereum blocks (the order has no meaning whatsoever, we just need some agreed-upon order) and reflected by the smart contract. Note that the order we used thus far is basically this order in a slight abuse of notation. Third, the public key $\gamma^{\xi_i}$ can also be used as an identifier of the participants.

% whenever communicating over Ethereum, the participants are asked to issue transactions from the Ethereum address with which they enrolled to the protocol. Other transactions are ignored. The participants are ordered according to their enrollment order and we denote them by their order $1,\dots, n$.            

% \item[\textit{Phase 2}] Commitments dissemination, from block $B_0+epoch+1$ to $B_0+2\cdot epoch$. In this phase the participants need to share their actual commitments between one another. While in the light version this was done over Ethereum, here the participants issue the very same transactions but instead of sending it to the Ethereum network they distribute them off-chain.

% \item[\textit{Phase 3}] Commitments verification, from block $B_+2\cdot epoch+1$ to $B_0+3\cdot epoch$. Each participant $i$ locally receives node $j$'s commitment transaction and verifies that (i) the commitments match the commitments Merkle root from the enrollment phase and that (ii) for all $0\leq k\leq t$ the following equalities hold:
% \begin{equation}
% \label{pairingCommitments}
% e\big(g_1,X^2_{j,k}\big)=e\big(X^1_{j,k},g_2\big)
% \end{equation}

% In particular, group membership is verified for each commitment, i.e., $\big( X^l_{j,k} \big)^q = \mathbb{I}_l$. If an equality does not hold for some $k$, then $i$ would forward $j$'s commitment transaction to the Ethereum network together with a complaint transaction indicating whether the complaint refers to the commitments Merkle root (invokes $2n$ hash computations \red{can we reduce this?}) or to the pairing equations (invokes to pairing computations). The smart contract would repeat the necessary computation and rule.

% There is another problematic scenario here: what if node $i$ hasn't received a commitment transaction from node $j$ by the time the phase is about to end? For that we have the following phase.

% \item[\textit{Phase 4}] time-out. During the time-out phase nodes have the opportunity to
% complain of not hearing a certain commitment transaction.

% \item[\textit{Phase 2'}] Commitments over Ethereum. If during phase 4, a complaint against node $j$ has been made, she must respond by submitting her commitment transaction to Ethereum. If she fails to do so she is kicked out from the protocol, her deposit shared between the rest of the participants (\red{how exactly?}) and the smart contract terminates. If she does submit the transaction, phase 3 is repeated.

% \item[\textit{Phase 3'}] Commitments Verification over Ethereum.

% \item[\textit{Phase 5}] Sub-shares dissemination. Each participant $i$ computes privately the values $x_{i,j}:=f_i(j)$ for every $j\neq i$, and sends $x_{i,j}$ to node $j$ off-chain. encrypts each of them using the encryption scheme explained in Sec.~\ref{DHXOR}, namely $e_{i,j}:=x_{i,j} \oplus  H\big(\gamma^{\xi_i\cdot \xi_j}\big)$. It then sends a transaction containing the data $\{e_{ij}\}_{j\ne i}$.

% \item[\textit{Phase 6}] Sub-share verification. Each participant $j$ privately verifies that the shares she received from participant $i$ are compatible with the public commitment made by $i$, by checking that the following equality hold: 
% \begin{equation}
% \label{shareVerification1}
% g_1^{x_{i,j}}=\prod_{k=0}^t \big(X^1_{i,k}\big)^{j^k}
% \end{equation}

% If some equality does not hold, $j$ files an \textit{invalid share} complaint, sending an Ethereum transaction specifying the identity $i$ for whom the equation did not hold, together with node $i$'s sub-share transaction. At this point, Ethereum would rerun the computation and rule.

% As in the commitment dissemination phase, also here the dissemination of some of the sub-shares transactions might fail. We employ the same type of time-out as in phase 4.

% \item[\textit{Phase 7}] time-out. During another time-out phase nodes have the opportunity to complain of not hearing a certain sub-share transaction.

% \item[\textit{Phase 5'}] Sub-shares dissemination over Ethereum. Any node that has been filed a complaint against during phase 7, must submit her relevant sub-share transaction, only this time it must be encrypted \red{(we can add the specific details of how the encryption is done)}, such that only the addressee may decrypt it.

% A node that fails to submit such a transaction is slashed, with the termination of the smart contract.
            
% \item[\textit{Phase 6'}] Sub-share verification over Ethereum. Phase 6 is repeated and complaints against invalid sub-shares filed. In order for the smart contract to be able to verify the computation in Equation~\ref{shareVerification1}, the complainer submits her secret decryption key together with her complaint.

% If no complaint transaction has been submitted during this phase, the protocol has finished successfully. Otherwise, the Ethereum smart contract would execute the relevant transaction and rule. 

% \item[\textit{Phase 8}]
% Each participant $j$ computes privately her final share $x_j:=\sum_i x_{ij}=\sum_i f_i(j)=:f(j)$.

% \item[\textit{Phase 9}] 
% Any participant can send a transaction specifying the public key obtained by the protocol, namely $X^2_0:=\prod_i X^2_{i,0}=\prod_i g_2^{f(0)}$ \red{(this needs more work to support complaints)}. Anyway, a \emph{termination transaction} is needed in order to return the deposits to all participants, and kill the contract.
% \end{itemize}

Complaints and framing should be designed ``Ethereum-compatible'', that is, the data and computation that they invoke must be reasonable within the Ethereum constraints. In general, this could be mitigated using interactive techniques between the ``accuser'' and the ``accused'' as in \red{cite TrueBit and Arbitrum}.    

\paragraph{Complaints}
The main goal of the complaint mechanism is to make sure that the sub-shares nodes communicate match the commitments they publish (phase $5$). The rest of the complaints deal with practical concerns which arise from using Ethereum and implementing the protocol in practice. To accommodate the single complaint philosophy, the complaints must be ``rulable'' in the sense that the smart contract can execute a computation and determine who is to blame. In the ``on-chain'' version, for clarity of presentation, this is done rather naively, not minimizing on-chain data usage or computation. Since the complexity of the computations needed to rule depends on $n$ and $t$ \red{(linearly? quadratically?)}, this approach is impractical when $n$ is large \red{reference gas costs graphs}. The ``off-chain'' protocol deals with such concerns, mitigating expensive usage of Ethereum.

The complaints are rather straightforward and always have two sides---the \emph{accuser} and the \emph{accused}. They deal with two types of misconducts---failing to submit a transaction in time or submitting a transaction with invalid data. In the first case, no computation is required from the smart contract\footnote{Note that in the ``off-chain'' version, this type of complaints becomes more complicated as Ethereum cannot determine whether information was exchanged off-chain. To resolve this difficulty, the ``off-chain'' protocol falls back to Ethereum and requires the ``accused'' participant to submit the data on-chain. This should be a very rare scenario.}. In the second case, if an additional piece of data is required for the smart contract to rule, it must be included in the complaint\footnote{In the ``off-chain'' version, the expensive complaints are dealt with using an interactive protocol (over Ethereum) between the ``accuser'' and the ``accused''. This way the dispute mechanism may be kept cheap and scale with $n$.}.

The complaints should cover all misconducts possible in the protocol. Indeed, it is possible to design complaints for all possible misconducts, apart from two---``not complaining'' and collusion. 

In the next section we give an exhaustive list of \red{all} misconducts and show that apart from two, there are relevant complaints for. Any misconduct for which there is a corresponding complaint is highly improbable as it might invoke someone complaining, slashing the accused's deposit. To deal with ``not complaining'' we motivate complaining with a reward. To deal with collusion, which is crucial for secrecy, we either assume a limited adversary or give the economic model which shows collusion is not rational (under realistic economic assumptions).     
  
Complaints or disputes, filed via \emph{complaint transactions}  They are divided to two kinds---``rulable'' and ``un-rulable'' (``un-rulable'' complaints are referred to as ``pings''). In the first kind, all the state needed for Ethereum to ``rule'' is included in the complaint transaction and a final call is made by Ethereum. In the second case, a special phase begins, by the end of which, the accused has to transmit a \emph{response transaction} that may keep the protocol alive. We don't get into the details of the complaint mechanism just yet, only emphasize that while complaints are regarded as cheap communication in GJKR, we must regard them as expensive and try to avoid them. Thus, we result in a zero-tolerant complaint mechanism. 

\red{Let's try to incorporate the complaints into the protocol description.}
We denote by $copm^l_{j,i}$ the complaint on item $1\leq l\leq 6$ in \ref{FaultyList} made by $j$ against $i$. If a participant filed an unjustified complaint (item $7$ in the list), no complaint is needed - the smart contract would detect this misconduct independently. The complaints contain the complaint type, as well as the following data: 
\begin{enumerate}
\item $copm^1_{j,i}$ No additional data. 
\item $copm^2_{j,i}$ No additional data.
\item $copm^3_{j,i}$ When complaining on $X^u_{i,k_0}$, include $u,k_0,$ and the signed commitments transaction $i$ sent $j$, \red{($i$ sent this transaction to everybody)}. 
\item $copm^4_{j,i}$ Include the signed commitments transaction $i$ sent $j$.
\item $copm^5_{j,i}$ Include the signed commitments transaction $i$ sent $j$.
\item $copm^6_{j,i}$ Include the signed commitments transaction $i$ sent $j$, as well as the one of the following: a (signed by $i$) transaction including the subshare, or else $j$-s private encryption key $\xi_j$.
\end{enumerate}

\paragraph{Framing}
There are two types of framings---revealing absolute secrets and revealing secrets prior to some \red{predetermined target time}. Framing can be targeted towards specific participants or towards the entire network. In general, it is most profitable (for the colluding parties) and disturbing (for ``the public'' or the users of the cryptosystem) to obtain full control of the system and thus someone that frames the whole network should be rewarded significantly, with $t\cdot D$ Eth (the rest is burnt). For a possible framer to refrain from framing she should be in a state where she can lose more than $t\cdot D$ if she does frame. If such an amount is highly improbable for someone to risk relative to the amount she might gain from controlling the cryptosystem, it can be seen as crypto-economically secure. We analyze a specific system to demonstrate this principle in Sec.~\ref{}.    

\paragraph{Analogy to the prisoner's dilemma}
In essence we build a scenario that is equivalent to the prisoner's dilemma---a given colluder's best strategy is to frame her peers no matter what they do. If they choose not to frame her, she is better off framing them (as long as $t\cdot D >\frac{Reward}{t+1} \cdot risk$) and if they do frame her she is of course better off framing them in the hope her frame would be processed first. Two pointers: In order to complicate their interests, the colluders can put themselves in a position where they risk more than $t\cdot D$ in case they choose to frame to once again overturn the interest balance. Thus, for a such a threshold crypto-system to be regarded as crypto-economically secure one should believe $t\cdot D$ is an unfeasible amount to deposit/put at risk or that it is not worth it investment wise.   










